Termite: A System for Tunneling Through Heterogeneous Data

Data-driven analysis is important in virtually every modern organization. Yet, most data is underutilized because it remains locked in silos inside of organizations; large organizations have thousands of databases, and billions of files that are not integrated together in a single, queryable repository. Despite 40+ years of continuous effort by the database community, data integration still remains an open challenge. In this paper, we advocate a different approach: rather than trying to infer a common schema, we aim to find another common representation for diverse, heterogeneous data. Specifically, we argue for an embedding (i.e., a vector space) in which all entities, rows, columns, and paragraphs are represented as points. In the embedding, the distance between points indicates their degree of relatedness. We present Termite, a prototype we have built to learn the best embedding from the data. Because the best representation is learned, this allows Termite to avoid much of the human effort associated with traditional data integration tasks. On top of Termite, we have implemented a Termite-Join operator, which allows people to identify related concepts, even when these are stored in databases with different schemas and in unstructured data such as text files, webpages, etc. Finally, we show preliminary evaluation results of our prototype via a user study, and describe a list of future directions we have identified.

==> sections/relemb2.tex <==
\section{Learning the Embedding}
\label{sec:relemb}

In this section, we first describe how we learn the embedding (Component 3 in
\F\ref{fig:overview} and Section~\ref{subsec:model}), how to refine it
(Component 4 in the figure and Section~\ref{subsec:refinement}), and how to
query it with the \emph{Termite-Join} operator, in
Section~\ref{subsec:termitejoin}.

\subsection{Deep Metric Learning}
\label{subsec:model}

Existing methods aim to learn the latent variables that \emph{explain}
observable data, \eg triples from a knowledge base~\cite{rescal, neuraltensor,
transe}, and use them for knowledge base completion among others.  Our goal is
different. We want to learn a deep metric for databases and text, because it
allows us to relate data to each other. 

\mypar{Setting}Our goal is to construct an embedding in which two related
entities represented by vectors $x_i$ and $x_j$ are closer to each other than to
a third, unrelated vector $x_k$. The training data is constructed as explained
in the previous section and consists of pairs of related and unrelated entities,
that are derived from triples extracted from text and relational data.  

\emph{Although in this first iteration we learn the deep metric from pairs of triples,
our ongoing research is centered in leveraging all the information represented
in relational data.}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.8\columnwidth]{img/siamesenetwork}
\caption{Architecture of the siamese network}
\label{fig:siamesenetwork}
\end{figure}

\mypar{Model Architecture} To learn the embedding, we need a {\it loss
function} that captures our optimization criteria. In particular, we want a higher loss (cost)
when two related vectors are far in the embedding, and when two unrelated
vectors are close to each other. This means we need a network architecture: 1)
that accepts two input vectors, \ie the input pair; 2) that can learn an
embedding representation for the input vectors and measure their distance; and
3) that can use that distance to compute the loss.

We use a Siamese network \cite{siamesenetwork, siamese} for learning the
embedding. Siamese networks are composed of two identical networks that share
weights, \textbf{input1} and \textbf{input2} in \F\ref{fig:siamesenetwork}).
Each training pair is fed to the network \eg say \textbf{input1} takes $x_i$ and
\textbf{input2} takes $x_j$. Each network transforms the input vector through
the four stacked layers, which are parameterized with the weights $w$. The
output of the fourth layer is the vectors' embedding representation, $f(x_i)$
and $f(x_j)$. The two networks connect in the loss layer, carrying the two
vector representations as well as the ground truth label, $Y$, that indicates
whether they are related ($Y=0$) or not, $Y=1$.

The loss layer is a contrastive
%\srm{citation or define or omit -- I don't know what this word means, nor will other readers} 
function~\cite{siamese}, $L$, defined as:

$$L(w, Y, f(x_i), f(x_j)) = (1 - Y)(Y')^2 + Y * (m - Y')^2$$

$Y'$ is the predicted output, which depends on $w$ and on the Euclidean distance
between $f(x_i)$ and $f(x_j)$. $m$ is a margin that enforces a minimum separation
between vectors in the embedding.

At first, $w$ is random, so the embedding vectors, $f(x_i)$ and $f(x_j)$
are placed randomly on the embedding. We use backpropagation and stochastic
gradient descent to learn $w$ and $f()$, the embedding that this component
produces as output.

\subsection{Refining the Embedding}
\label{subsec:refinement}

The learned embedding will contain anomalies: vectors
that are close together but are unrelated. This is because we only use a limited
number of negative samples during training and because of the curse of
dimensionality. If we leave the embedding untouched, we will produce wrong
results when querying it.

The refinement component (see number 4 in \F\ref{fig:overview}) modifies the
embedding and creates metadata to compensate for those anomalies during query
time. We explain the techniques implemented in Termite today as well as an
ongoing effort:

\mypar{Distance concentration and hubness} As data dimensionality increases (we
use 100-dimension vectors), all points tend to have the same distance to each
other~\cite{distanceconcentration}, a problem known as \emph{distance
concentration}. This is clearly at odds with our goal of using distance to
measure how related are data. To ameliorate this problem, we use cosine
distance at query time---despite building the embedding using Euclidean distance
in the loss function. We have also tried using fractional distances but they are
computationally more expensive and we do not observe an accuracy benefit.

\emph{Hubness} is the tendency of certain points to be close to many other points.
This is an even worse problem than distance concentration because it means that
certain data will be artificially related (close) to a lot of other data, which is directly
against the quality metric we desire for our embedding.

The good news is that we can largely ameliorate this problem.  The main
intuition of our technique is that it is possible to compute a \emph{hubness
factor} for each entity represented in the embedding, and then remove
entities with a high hubness factor in the top-k results. In
particular, we compute how many times each point appears close to other points
in the embedding. We then take the 75 percentile of the number of appearances as
a cutoff parameter. On query time, we filter out those entities of the top-k
results with a hubness factor higher than the cutoff parameter and pad the
ranking with additional entities until we have K elements. Empirically, this
improves the quality of the returned rankings.

\mypar{Topological data analysis} Once the embedding is built, it seems
intuitively interesting to understand shapes: which sets of points are strongly
related to each other. Whether two or more points are related---whether they
have a shape---boils down to determining if they are within a specific distance
of each other. Then, if they remain close as the distance grows, it is possible
to determine the strength of the relationship.  Using the same intuition, points
that do not remain close may be categorized as noise. Topological data analysis
(TDA) is a mathematical tool that permits reasoning about shapes in
high-dimensions algebraically. A central concept in TDA is persistent homology,
which indicates which shapes remain in the high-dimensional embedding as the
distance changes. A straightforward application of persistent homology to our
embedding gives us a degree of confidence for each of the results of the top-k
list, depending on how \emph{persistent} they are in the embedding. We are
currently investigating additional applications of the technique, as well as how
to best use TDA to curate the embedding.

\subsection{Termite-Join Operator}
\label{subsec:termitejoin}

Given an input entity, \emph{Termite-Join} returns the $K$ closest entities in the
embedding. All entities representations in the embedding are computed offline by
feeding the entities to the learned network and obtaining their representation.

At query time, given an input query $x_i$: 1) Obtain the embedding
representation, $f(x_i)$ from the collection. 2) Retrieve the $K$-closest
vectors to $f(x_i)$ from the collection. 3) Remove each $k_i \in K$ whose
hubness factor is beyond the cutoff parameter computed by the refinement
component. 4) Fill in the top-K list if some element has been removed in step 3.
5) Obtain the string representation of the top-k vectors and present the results
to the user.




==> tables/entity_table.tex <==
\begin{table*}[]
\small
\centering
\caption{Results for record linkage}
\label{table:entity_table}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\#Entities} & \textbf{\begin{tabular}[c]{@{}c@{}}Stats. per \\ entity \\
(min, avg, max)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\#
Alternative\\ entities\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Found\\ 1st query\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}\% Found\\ 1st query\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Found\\ 2nd query\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}\% Found\\ 2nd query\end{tabular}} \\ \hline
52                  & 2/4/7
& 210                                                                        &
156                                                                &
\textbf{74\%}                                                         & 163
& \textbf{77.6\%}                                                       \\
\hline
\end{tabular}
\end{table*}



